Tangent points of lower content $d$-regular sets and $\beta$ numbers

Given a lower content $d$-regular set in $\mathbb{R}^n$, we prove that the subset of points in $E$ where a certain Dini-type condition on the so-called Jones $\beta$ numbers holds coincides with the set of tangent points of $E$, up to a set of $\mathcal{H}^d$-measure zero. The main point of our result is that $\mathcal{H}^d|_E$ is not assumed to be $\sigma$-finite; because of this, we use a certain variant of the $\beta$ coefficient, firstly introduced by Azzam and Schul in [AS1], which is given in terms of integration with respect to the Hausdorff content.

==> 06_biblio.tex <==
\begin{thebibliography}{5}
\makeatletter
\renewcommand\@biblabel[1]{[AS1]}
\makeatother

\bibitem{azzam} 
Azzam J, Schul R. An analyst's traveling salesman theorem for sets of dimension larger than one. \textit{Mahtematische Annalen}, accepted 2017. Present on the ArXiv.

\makeatletter
\renewcommand\@biblabel[1]{[AT1]}
\makeatother

\bibitem{azzamtolsa} 
Azzam J, Tolsa X. Characterization of n-rectifiability in terms of Jones’ square function: Part II. \textit{Geometric and Functional Analysis}. 2015 Oct 1;25(5):1371-412.

\makeatletter
\renewcommand\@biblabel[1]{[Bes]}
\makeatother

\bibitem{besi}
Besicovitch AS. On the fundamental geometrical properties of linearly measurable plane sets of points. Mathematische Annalen. 1928 Mar 1;98(1):422-64.

\makeatletter
\renewcommand\@biblabel[1]{[BJ1]}
\makeatother

\bibitem{bishop} 
Bishop CJ, Jones PW. Harmonic measure, L 2-estimates and the Schwarzian derivative. \textit{Journal d'Analyse Mathématique}. 1994 Dec 1;62(1):77-113.

\makeatletter
\renewcommand\@biblabel[1]{[BS1]}
\makeatother

\bibitem{badger1} 
Badger M, Schul R. Multiscale analysis of 1-rectifiable measures: necessary conditions. \textit{Mathematische Annalen}. 2015 Apr 1;361(3-4):1055-72.

\makeatletter
\renewcommand\@biblabel[1]{[BS2]}
\makeatother

\bibitem{badger2} 
Badger M, Schul R. Two sufficient conditions for rectifiable measures. \textit{Proceedings of the American Mathematical Society}. 2016;144(6):2445-54.

\makeatletter
\renewcommand\@biblabel[1]{[BS3]}
\makeatother

\bibitem{badger3} 
Badger M, Schul R. Multiscale analysis of 1-rectifiable measures II: characterizations. \textit{Analysis and Geometry in Metric Spaces}. 2017 Mar 1;5(1):1-39.

\makeatletter
\renewcommand\@biblabel[1]{[Ch1]}
\makeatother

\bibitem{christ}
Christ M. A T(b) Theorem with remarks on analytic capacity and the Cauchy integral. \textit{Colloquium Mathematicum}, 1990.

\makeatletter
\renewcommand\@biblabel[1]{[CW1]}
\makeatother

\bibitem{cw1}
Cs\"{o}rnyei, M. and Wilson, B. Tangents of $\sigma$-finite curves and scaled oscillation. \textit{Math. Proc. Cambr. Phil. Soc.}, vol. 161, no. 1, (2014), 1-12.

\makeatletter
\renewcommand\@biblabel[1]{[Da1]}
\makeatother

\bibitem{da1}
David G. Morceaux de graphes lipschitziens at integrales singulieres sur une surface. \textit{Rev. Mat. Iberoamericana}, 1998.

\makeatletter
\renewcommand\@biblabel[1]{[Do1]}
\makeatother

\bibitem{do1}
Dorronsoro JR. A characterization of potential spaces. Proceedings of the American Mathematical Society. 1985;95(1):21-31.

\makeatletter
\renewcommand\@biblabel[1]{[DS1]}
\makeatother

\bibitem{ds1}
David G, Semmes S. Singular integrals and rectifiable sets in Rn: Au-dela des graphes lipschitziens. \textit{Asterisque}; 1991

\makeatletter
\renewcommand\@biblabel[1]{[DS2]}
\makeatother

\bibitem{ds2}
David G, Semmes S. \textit{Analysis of and on uniformly rectifiable sets}. American Mathematical Society; 1993.

\makeatletter
\renewcommand\@biblabel[1]{[DT1]}
\makeatother

\bibitem{davidtoro} 
David G, Toro T. Reifenberg parameterizations for sets with holes. \textit{Memoirs of the American Mathematical Society}. 2012.

\makeatletter
\renewcommand\@biblabel[1]{[EG1]}
\makeatother

\bibitem{evans}
Evans LC, Gariepy RF. \textit{Measure theory and fine properties of functions}. CRC press; 2015 Apr 17.

\makeatletter
\renewcommand\@biblabel[1]{[ENV1]}
\makeatother

\bibitem{naber}
Edelen, N., Naber, A. and Valtorta, D., 2016. Quantitative Reifenberg theorem for measures. arXiv preprint arXiv:1612.08052.

\makeatletter
\renewcommand\@biblabel[1]{[Fa1]}
\makeatother

\bibitem{fang}
Fang, X. The Cauchy Integral of Calder\'{o}n and Analytic Capacity . Ph.D. dissertation (1990).

\makeatletter
\renewcommand\@biblabel[1]{[Fed]}
\makeatother

\bibitem{federer}
Federer H. \textit{Geometric measure theory}. Springer; 2014 Nov 25.

\makeatletter
\renewcommand\@biblabel[1]{[G1]}
\makeatother

\bibitem{ghinazzi}
Ghinassi, S. A sufficient condition for $C^{1, \alpha}$ parameterisation. 2017, ArXiv preprint.

\makeatletter
\renewcommand\@biblabel[1]{[He1]}
\makeatother

\bibitem{heinonen}
Heinonen, J. \textit{Lectures on Lipschitz analysis}. Unpublished.

\makeatletter
\renewcommand\@biblabel[1]{[HM1]}
\makeatother

\bibitem{hytonen} 
Hyt\"{o}nen T, Martikainen H. Non-homogeneous Tb theorem and random dyadic cubes on metric measure spaces. \textit{Journal of Geometric Analysis}. 2012 Oct 1;22(4):1071-107.

\makeatletter
\renewcommand\@biblabel[1]{[J1]}
\makeatother

\bibitem{jones} 
Jones PW. Rectifiable sets and the traveling salesman problem. \textit{Inventiones Mathematicae}, 1990.

\makeatletter
\renewcommand\@biblabel[1]{[L1]}
\makeatother

\bibitem{lerman} 
Lerman G. Quantifying curvelike structures of measures by using L2 Jones quantities. \textit{Communications on pure and applied mathematics}. 2003 Sep 1;56(9):1294-365.

\makeatletter
\renewcommand\@biblabel[1]{[LMR1]}
\makeatother

\bibitem{maggioni} 
Little, A.V., Maggioni, M. and Rosasco, L. Multiscale geometric methods for data sets I: Multiscale SVD, noise and curvature. \textit{Applied and Computational Harmonic Analysis.} 2016.

\makeatletter
\renewcommand\@biblabel[1]{[M1]}
\makeatother

\bibitem{mattila}
Mattila P. \textit{Geometry of sets and measures in Euclidean spaces: fractals and rectifiability}. Cambridge university press; 1999.

\makeatletter
\renewcommand\@biblabel[1]{[Ok1]}
\makeatother

\bibitem{oki}
Okikiolu, K. Characterization of subsets of rectifiable curves in Rn. \textit{Journal of the London Mathematical Society}. 1992.


\makeatletter
\renewcommand\@biblabel[1]{[P1]}
\makeatother

\bibitem{pajot}
Pajot, H. Conditions quatitatives de rectifiabilit\`{e}. \textit{Bull. Soc. Math. France}. 1997.

\makeatletter
\renewcommand\@biblabel[1]{[Sch1]}
\makeatother

\bibitem{sch1}
Schul, R. Subsets of rectifiable curves in Hilbert Space - the analyst's TSP. \textit{J. Anal. Math.}, 2007.

\makeatletter
\renewcommand\@biblabel[1]{[St1]}
\makeatother

\bibitem{stein}
Stein EM. \textit{Harmonic Analysis: Real-Variable Methods, Orthogonality, and Oscillatory Integrals}. Princeton University Press; 2016.

\makeatletter
\renewcommand\@biblabel[1]{[St2]}
\makeatother

\bibitem{stein2}
Stein EM. \textit{Stein EM. Singular integrals and differentiability properties of functions (PMS-30)}. Princeton university press.

\makeatletter
\renewcommand\@biblabel[1]{[T1]}
\makeatother

\bibitem{tolsa1}
Tolsa X. Characterization of n-rectifiability in terms of Jones’ square function: part I. \textit{Calculus of Variations and Partial Differential Equations}. 2015 Dec 1;54(4):3643-65.

\makeatletter
\renewcommand\@biblabel[1]{[T2]}
\makeatother

\bibitem{tolsa2}
Tolsa X. Rectifiability of measures and the $\beta_p$ coefficients. 2017, ArXiv preprint.

\end{thebibliography}
